A Variance-Reduced Stochastic Accelerated Primal Dual Algorithm

In this work, we consider strongly convex strongly concave (SCSC) saddle point (SP) problems $\min_{x\in\mathbb{R}^{d_x}}\max_{y\in\mathbb{R}^{d_y}}f(x,y)$ where $f$ is $L$-smooth, $f(.,y)$ is $\mu$-strongly convex for every $y$, and $f(x,.)$ is $\mu$-strongly concave for every $x$. Such problems arise frequently in machine learning in the context of robust empirical risk minimization (ERM), e.g. $\textit{distributionally robust}$ ERM, where partial gradients are estimated using mini-batches of data points. Assuming we have access to an unbiased stochastic first-order oracle we consider the stochastic accelerated primal dual (SAPD) algorithm recently introduced in Zhang et al. [2021] for SCSC SP problems as a robust method against gradient noise. In particular, SAPD recovers the well-known stochastic gradient descent ascent (SGDA) as a special case when the momentum parameter is set to zero and can achieve an accelerated rate when the momentum parameter is properly tuned, i.e., improving the $\kappa \triangleq L/\mu$ dependence from $\kappa^2$ for SGDA to $\kappa$. We propose efficient variance-reduction strategies for SAPD based on Richardson-Romberg extrapolation and show that our method improves upon SAPD both in practice and in theory.

==> [Arxiv] Variance Reduced SAPD-2/defs.tex <==
% MATH SUMBOLS AND RELATED MACROS
\def\grad{\nabla}
\def\noi{\noindent}
\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
%\def\bc{\mathbf{c}}
\def\bd{\mathbf{d}}
\def\be{\mathbf{e}}
\def\bff{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
\def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}  %{\mbox{\boldmath $\lambda$}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}
\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bU{\mathbf{U}}
\def\bT{\mathbf{T}}
\def\bY{\mathbf{Y}}
\def\bX{\mathbf{X}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bZ{\mathbf{Z}}
\def\bo{\mathbf{0}}

\def\e{{\boldsymbol{\epsilon}}}
\def\l{{\boldsymbol{\lambda}}}
\def\g{{\boldsymbol{\gamma}}}
\def\G{{\boldsymbol{\Gamma}}}
\def\L{{\boldsymbol{\Lambda}}}
\def\D{{\boldsymbol{\Delta}}}
\def\a{{\boldsymbol{\alpha}}}
\def\m{{\boldsymbol{\mu}}}
\def\n{{\boldsymbol{\nu}}}
%\def\S{{\boldsymbol{\Sigma}}}
\def\p{{\boldsymbol{\pi}}}
\def\th{{\boldsymbol{\theta}}}
\def\Th{{\boldsymbol{\Theta}}}
\def\x{{\boldsymbol{\xi}}}
\def\b{{\boldsymbol{\beta}}}
\def\r{{\boldsymbol{\rho}}}
\def\z{{\boldsymbol{\zeta}}}
\def\ph{{\boldsymbol{\phi}}}
\def\ps{{\boldsymbol{\psi}}}
\def\pis{\pi^{\star}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}



\def\mA{\mathbb{A}}
\def\mB{\mathbb{B}}
\def\mC{\mathbb{C}}
\def\mD{\mathbb{D}}
\def\mE{\mathbb{E}}
\def\mF{\mathbb{F}}
\def\mG{\mathbb{G}}
\def\mH{\mathbb{H}}
\def\mI{\mathbb{I}}
\def\mJ{\mathbb{J}}
\def\mK{\mathbb{K}}
\def\mL{\mathbb{L}}
\def\mM{\mathbb{M}}
\def\mN{\mathbb{N}}
\def\mO{\mathbb{O}}
\def\mP{\mathbb{P}}
\def\mQ{\mathbb{Q}}
\def\mR{\mathbb{R}}
\def\mS{\mathbb{S}}
\def\mT{\mathbb{T}}
\def\mU{\mathbb{U}}
\def\mV{\mathbb{V}}
\def\mW{\mathbb{W}}
\def\mX{\mathbb{X}}
\def\mY{\mathbb{Y}}
\def\mZ{\mathbb{Z}}

\def\eq{\[}
\def\en{\]}

\def\smskip{\smallskip}
\def\sep#1{ \hskip -5pt & #1 & \hskip -5 pt}
\def\texitem#1{\par\smskip\noindent\hangindent 25pt
               \hbox to 25pt {\hss #1 ~}\ignorespaces}

% mathematical constructs
\def\abs#1{\left|#1\right|}
\def\norm#1{\|#1\|}
\def\vec#1{\left(\!\begin{array}{c}#1\end{array}\!\right)}
\def\bmat#1{\left[\begin{array}{cc}#1\end{array}\right]}

% some traditional definitions that can be blamed on craig barratt
\newcommand{\BEAS}{\begin{eqnarray*}}
\newcommand{\EEAS}{\end{eqnarray*}}
\newcommand{\BEA}{\begin{eqnarray}}
\newcommand{\EEA}{\end{eqnarray}}
\newcommand{\BEQ}{\begin{eqnarray}}
\newcommand{\EEQ}{\end{eqnarray}}
\newcommand{\BIT}{\begin{itemize}}
\newcommand{\EIT}{\end{itemize}}
\newcommand{\BNUM}{\begin{enumerate}}
\newcommand{\ENUM}{\end{enumerate}}

% arash added these two
\newcommand{\BA}{\begin{array}}
\newcommand{\EA}{\end{array}}

% text abbrevs
\newcommand{\cf}{{\it cf.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it etc.}}

\newcommand{\ones}{\mathbf 1}

% std math stuff
\newcommand{\reals}{\mathbb{R}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\eqbydef}{\mathrel{\stackrel{\Delta}{=}}}
\newcommand{\complex}{\mathbb{C}}

% Re & Im
%\renewcommand{\Re}{\mathop{\bf Re}}
%\renewcommand{\Im}{\mathop{\bf Im}}

% lin alg stuff
\newcommand{\Span}{\mbox{\textrm{span}}}
%\newcommand{\Range}{\mbox{\textrm{range}}}
\newcommand{\nullspace}{{\mathcal N}}
\newcommand{\range}{{\mathcal R}}
\newcommand{\Nullspace}{\mbox{\textrm{nullspace}}}
\newcommand{\Rank}{\mathop{\bf rank}}
\newcommand{\Tr}{\mathop{\bf Tr}}
\newcommand{\detr}{\mathop{\bf det}}
%\newcommand{\diag}{\mathop{\bf diag}}
\newcommand{\lambdamax}{{\lambda_{\rm max}}}
\newcommand{\lambdamin}{\lambda_{\rm min}}

% probability stuff
\newcommand{\Expect}{\mathop{\bf E{}}}
\newcommand{\Prob}{\mathop{\bf Prob}}
\newcommand{\erf}{\mathop{\bf erf}}
\def\Pr{\mathbb{P}}

% convexity & optimization stuff
\def\co{{\mathop {\bf cone}}}
\def\conv{\mathop {\bf conv}}
%\def\var#1{\mathop{\bf Var}\big[#1\big]}
\newcommand{\dist}{\mathop{\bf dist{}}}
\newcommand{\Ltwo}{{\bf L}_2}

%\newcommand{\QED}{~~\rule[-1pt]{8pt}{8pt}}\def\qed{\QED}
%\newcommand{\approxleq}{\mathrel{\smash{\makebox[0pt][l]{\raisebox{-3.4pt}{\small$\sim$}}}{\raisebox{1.1pt}{$<$}}}}
\newcommand{\epi}{\mathop{\bf epi}}
\newcommand{\hypo}{\mathop{\bf hypo}}
\newcommand{\ri}{\mathop{\bf ri}}
\newcommand{\vol}{\mathop{\bf vol}}
\newcommand{\Vol}{\mathop{\bf vol}}

\newcommand{\dom}{\mathop{\bf dom}}
\newcommand{\aff}{\mathop{\bf aff}}
\newcommand{\cl}{\mathop{\bf cl}}
\newcommand{\Angle}{\mathop{\bf angle}}
\newcommand{\intr}{\mathop{\bf int}}
\newcommand{\relint}{\mathop{\bf rel int}}
\newcommand{\bdry}{\mathop{\bf bd}}
\newcommand{\vect}{\mathop{\bf vec}}
\newcommand{\dsp}{\displaystyle}
\newcommand{\foequal}{\simeq}
\newcommand{\VOL}{{\mbox{\bf vol}}}

%the following ones seem way too specialized to be here...
\newcommand{\xopt}{x^{\rm opt}}
\newcommand{\Xb}{{\mbox{\bf X}}}
\newcommand{\xst}{x^\star}
\newcommand{\varphist}{\varphi^\star}
\newcommand{\lambdast}{\lambda^\star}
\newcommand{\Zst}{Z^\star}
\newcommand{\fstar}{f^\star}
\newcommand{\xstar}{x^\star}
\newcommand{\xc}{x^\star}
\newcommand{\lambdac}{\lambda^\star}
\newcommand{\lambdaopt}{\lambda^{\rm opt}}

%generalized inequalities for cvx book
\newcommand{\geqK}{\mathrel{\succeq_K}}
%\newcommand{\geqq}{\mathrel{\succeq_{\cQ}}}
\newcommand{\gK}{\mathrel{\succ_K}}
\newcommand{\leqK}{\mathrel{\preceq_K}}
\newcommand{\lK}{\mathrel{\prec_K}}
\newcommand{\geqKst}{\mathrel{\succeq_{K^*}}}
\newcommand{\gKst}{\mathrel{\succ_{K^*}}}
\newcommand{\leqKst}{\mathrel{\preceq_{K^*}}}
\newcommand{\lKst}{\mathrel{\prec_{K^*}}}
\newcommand{\geqL}{\mathrel{\succeq_L}}
\newcommand{\gL}{\mathrel{\succ_L}}
\newcommand{\leqL}{\mathrel{\preceq_L}}
\newcommand{\lL}{\mathrel{\prec_L}}
\newcommand{\geqLst}{\mathrel{\succeq_{L^*}}}
\newcommand{\gLst}{\mathrel{\succ_{L^*}}}
\newcommand{\leqLst}{\mathrel{\preceq_{L^*}}}
\newcommand{\lLst}{\mathrel{\prec_{L^*}}}
\def\join{\vee}
\def\meet{\wedge}

% colored text
\def\red#1{\textcolor{red}{#1}}
\def\green#1{\textcolor{green}{#1}}
\def\blue#1{\textcolor{blue}{#1}}
\def\tri#1{\textcolor{#1}{$\blacktriangleright$}}

%% macros

\newif\ifpagenumbering
\pagenumberingtrue
\newcommand{\firstpagenumber}{1}
\pagenumberingfalse

%
%  Conditionals for generating different versions
%
% \newif\ifabstract
% \newif\ifjournal
% \newcommand{\mnote}[1]{{\tiny\marginpar[#1]{#1}}}
\newsavebox{\theorembox}
\newsavebox{\lemmabox}
% \newsavebox{\claimbox}
% \newsavebox{\factbox}
\newsavebox{\defnbox}
% \newsavebox{\corollarybox}
% \newsavebox{\propositionbox}
% \newsavebox{\examplebox}
% \newsavebox{\exercisebox}
% \newsavebox{\problembox}
% \newsavebox{\conjecturebox}
% \newsavebox{\oqbox}
%\newsavebox{\remarkbox}
\newsavebox{\assbox}
\savebox{\theorembox}{\noindent\bf Theorem}
\savebox{\lemmabox}{\noindent\bf Lemma}
% \savebox{\claimbox}{\noindent\bf Claim}
% \savebox{\factbox}{\noindent\bf Fact}
\savebox{\defnbox}{\noindent Definition}
% \savebox{\corollarybox}{\noindent\bf Corollary}
% \savebox{\propositionbox}{\noindent\bf Proposition}
% \savebox{\examplebox}{\noindent\bf Example}
% \savebox{\exercisebox}{\noindent\bf Exercise}
% \savebox{\problembox}{\noindent\bf Problem}
% \savebox{\conjecturebox}{\noindent\bf Conjecture}
%\savebox{\remarkbox}{\noindent\bf Remark}
% \savebox{\oqbox}{\noindent\bf Open Question}
%\savebox{\assbox}{\noindent\bf Assumption}
%\newtheorem{assumption}{\usebox{\assbox}}
%\newtheorem{theorem}{\usebox{\theorembox}}
%\newtheorem{lemma}{\usebox{\lemmabox}}
% \newtheorem{claim}{\usebox{\claimbox}}
% \newtheorem{fact}{\usebox{\factbox}}
%\newtheorem{remark}{\usebox{\remarkbox}}[section]
% \newtheorem{corollary}{\usebox{\corollarybox}}
% \newtheorem{proposition}[theorem]{\usebox{\propositionbox}}
% \newtheorem{exercise}{\usebox{\exercisebox}}
% \newtheorem{example}{\usebox{\examplebox}}
% \newtheorem{problem}{\usebox{\problembox}}
% \newtheorem{conjecture}{\usebox{\conjecturebox}}
% \newtheorem{oq}{\usebox{\oqbox}}
\newtheorem{defn}{\usebox{\defnbox}}
\def\blackslug{\hbox{\hskip 1pt \vrule width 4pt height 8pt depth 1.5pt
\hskip 1pt}}
%\newtheorem{exprime}{Example}%[section]
%\newenvironment{example}{\noindent\exprime\em {\vspace{-0.05 in}}}{
%\hfill $\blackslug$ \par \addvspace{\bigskipamount}{\vspace{0in}}}
%% \newenvironment{example}{\noindent\exprime\em {\vspace{-0.05 in}}}{
%% \hfill $\blackslug$ \par \addvspace{\bigskipamount}{\vspace{0in}}}

%Miscellaneous commands for proofs
%\newcommand{\qed}{\mbox{}\hspace*{\fill}\nolinebreak\mbox{$\rule{0.7em}{0.7em}$}}
\newcommand{\proc}[1]{\textnormal{\scshape#1}}
\usepackage{soul}
%\newenvironment{proof}{\par{\noi \bf Proof: }}{\(\qed\) \par}
% \newenvironment{proofsketch}{\par{\noi \bf Proof Sketch:}}{\(\qed\) \par}
% \newenvironment{solutionsketch}{\par{\bf Solution Sketch:}}{\(\qed\) \par}
% \newenvironment{deffproof}[1]{\par{\bf Proof #1:}}{\(\qed\) \par}
% \newcommand{\case}[1]{{\small \sc Case #1:}}
% \newcommand{\subcase}[1]{{\em Case #1:}\/}

% \renewcommand{\hat}[1]{\widehat{#1}}
% \newcommand{\opt}{\mbox{\footnotesize\sc opt}}
% \newcommand{\parent}{\mbox{\sc parent}}
% \newcommand{\precstar}{\stackrel{\mbox{\raisebox{-0.5ex}[0pt][0pt]{\tiny$\star$}}}{\prec}}

\usepackage[normalem]{ulem}
\DeclareUnicodeCharacter{2212}{~}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> [Arxiv] Variance Reduced SAPD-2/notations_and_packages.tex <==

% added by us
\usepackage{amsmath,amsthm,amsfonts,amssymb}
\usepackage{enumerate,color,xcolor}
\usepackage{url}
\usepackage[utf8]{inputenc}

\newcommand{\bc}[1]{{\color{blue} #1}}
\newcommand{\bcred}[1]{{\color{orange} #1}}
%added by us
\newtheorem{theorem}{Theorem}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{condition}{Condition}
\newtheorem{example}{Example}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{notation}{Notation}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{question}{Question}
\newtheorem{remark}{Remark}
%\newcommand{\remark}{\noindent {\bf Remark. }}[section]
\newtheorem{assumption}{Assumption}

%Added by NSA 04/16/21
\usepackage{todonotes}
\def\sa#1{\textcolor{red}{#1}}
\def\fprod#1{\left\langle#1\right\rangle}
\def\prox#1{\mathbf{prox}_{#1}}
\def\nsa#1{\todo[inline, size=footnotesize]{NSA:~#1}}
\newcommand{\vertiii}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

%Added by BC 05/10/21 
\newcommand{\Pk}{\mathcal{P}_k}
\newcommand{\mP}{\mathcal{P}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\mN}{\mathbb{N}}
\newcommand{\mR}{\mathbb{R}^d}
\newcommand{\mRx}{\mathbb{R}^{d_x}}
\newcommand{\mRy}{\mathbb{R}^{d_y}}
\newcommand{\tPhi}{\tilde{\Phi}}
\newcommand{\veps}{w}
\newcommand{\mW}{\mathcal{W}}
\newcommand{\tn}{\tilde{\nabla}}
\newcommand{\cn}{{\color{red}[Citation Needed]}}
\newcommand{\mcR}{\mathcal{R}}
\newcommand{\mbR}{\mathbf{R}}
\newcommand{\omgx}{\omega^{x}}
\newcommand{\omgy}{\omega^{y}}
% \newcommand{\ztdt}{z^{(\tau,\delta,\theta)}}
\newcommand{\xitdt}{\xi^{(\tau,\sigma,\theta)}}
\newcommand{\ptdt}{\pi^{(\tau,\sigma,\theta)}}
\newcommand{\mRd}{\mathbb{R}^d}
\newcommand{\mcRtdt}{\mathcal{R}^{(\tau,\sigma,\theta)}}
\newcommand{\mcRa}{\mathcal{R}^{(\alpha)}}
\newcommand{\Epi}{\mathbb{E}_{\pi_\infty}}
\newcommand{\pa}{\pi^{(\alpha)}}
\newcommand{\za}{z^{(\alpha)}}
\newcommand{\zt}{z^{(\theta)}}
\newcommand{\xit}{\xi^{(\theta)}}
\newcommand{\mE}{\mathbb{E}_{\pi^{(\theta)}_*}}
\newcommand{\hes}{\nabla^{(2)}f_*}
\newcommand{\mV}{\mathcal{V}}
\newcommand{\gV}{\cV^{(\tau,\sigma,\theta)}_\alpha}

==> [Arxiv] Variance Reduced SAPD-2/sections/introduction.tex <==
\section{Introduction}\label{sec: introduction}
\mg{Saddle point (SP) problems arise frequently in many key settings in machine learning. Examples include but are not limited to robust training of machine learning models \cite{gurbuzbalaban2020stochastic,duchi2021learning}, training Generative Adversarial Networks (GANs) \cite{pmlr-v70-arjovsky17a}, design of fair classifiers \cite{nouiehed2019solving}, and empirical risk minimization~(ERM) problems such as regression and classification \cite{palaniappan2016stochastic}. \sa{Furthermore, ERM problems} with constraints on the model parameters result in constrained stochastic optimization problems which can also be cast into saddle-point problems %based on 
\sa{using} Lagrangian duality.} %optimization 

\mg{Motivated by such applications, we consider the strongly convex/strongly concave~\sa{(SCSC)} saddle-point~\sa{(SP)} problem
\begin{equation}\label{def: sapd-opt-prob}
    \min_{x\in \mRx}\max_{y\in\mRy} \; f(x,y),
\end{equation}
where $f:\mathbb{R}^{d_x}\times \mathbb{R}^{d_y} \to \mathbb{R}$ is smooth and strongly convex %with respect to 
\sa{in} $x$ and strongly \sa{concave} %with respect to 
\sa{in} $y$. As we discuss in the numerical experiments section, our algorithms and results are also directly applicable to the convex/concave setting by adding an appropriate quadratic regularizer. \sa{In a different setting, SCSC problems of the form given in \eqref{def: sapd-opt-prob} arise as subproblems when solving weakly convex-weakly concave SP problems using inexact proximal point method, e.g., see~\cite{liu2021first}}.

\sa{We consider \eqref{def: sapd-opt-prob} assuming we only have} access to unbiased stochastic estimates of the true gradients $\nabla_x f(x,y)$ and $\nabla_y f(x,y)$; as often in machine learning applications gradients are not exactly computed but \sa{are} estimated from randomly sampled subsets (mini-batches) of data.} This is also the case in privacy-preserving empirical risk minimization where noise is added to the gradients to preserve privacy of the user data \cite{chaudhuri2011differentially}. \mg{For solving these SP problems, stochastic first-order (SFO) methods that rely on stochastic gradient information have been very popular in practice due to their favorable scalability properties\sa{; but,} they come with a number of challenges. In particular, even though the problem \eqref{def: sapd-opt-prob} is well-studied when the gradients are deterministic, many aspects of the stochastic setting with inexact gradient information are relatively understudied.
%\sa{e.g., see the references in~\cite{zhang2021robust}.
%\sa{except for some} special cases such as bilinear SP problems \cite{zhang2021robust}. 
In fact, accelerated SFO methods \sa{achieving} acceleration beyond bilinear problems are quiet recent in the literature, e.g., \cite{accSFO_SP_1, fallah_2020, zhang2021robust, VarRedSGLD,VarRedSpiderBoost,thekumparampil2019efficient,chen2017accelerated,hsieh2019convergence} and the references therein. To that end, the \sa{recently proposed} stochastic accelerated primal-dual \sa{(SAPD) method~\cite{zhang2021robust}, 
%is a recently proposed 
\sa{based on momentum-averaging,} 
%based accelerated method that 
can achieve the best iteration complexity bound among single-loop methods for SCSC problems of the form: $\min_x\max_yg(x)+f(x,y)-h(y)$, where $f$ is a smooth SCSC function admitting an SFO oracle as we assume for the SP problem in~\eqref{def: sapd-opt-prob}, and $g,h$ are closed, strongly convex functions with efficient proximal maps; furthermore, SAPD achieves the optimal complexity for bilinear SP problems with $f(x,y)=\fprod{Ax,y}$ for some $A\in\reals^{d_y\times d_x}$.} In particular, SAPD, \sa{which is an extension of the APD~\cite{hamedani2021primal} algorithm from deterministic to stochastic first-order oracle setting,} recovers the well-known stochastic gradient descent ascent (SGDA) as a special case when the momentum parameter is set to zero and can achieve an accelerated rate when the momentum parameter is properly tuned, \sa{i.e., improving the $\kappa\triangleq L/\mu$ dependence from $\kappa^2$ for SGDA to $\kappa$.}} 
 
%\notemg{Although bilinear case is better studied, the general case is more recent; the acc. alg. that can improve upon SGDA is recent. However, they suffer from increased variance as accelerated methods. Based on Romberg interpolation, we reduce the variance. Such techniques were used in non-accelerated primal methods.}
%\bc{[Why variance reduction techniques are important and what are the methods for that]}
%\notemg{need some references to the bib file about variance reduction for saddle-point algorithms, for example those designated for finite-sum problems}
%\notemg{Mention here why constant stepsize has some advantages, it is less parameters to tune compared to decaying stepsize$a/(b+ck)$. }
%\notemg{need to assume noise has 4th moment somewhere}
%\bc{[More motivation here]}
% In the literature, several algorithms have \sa{been} proposed to solve \sa{the SCSC %saddle point 
% SP problem in}~\eqref{def: sapd-opt-prob}. \bc{[The other known methods in the literature and their comparison]}. Considering the %large 
% \sa{sheer size of the problems arising in practice}, the \sa{first-order} methods which only require first-order information, i.e., the gradient of \sa{$f$, %the objective, 
% have become the method of choice as they are more efficient to implement}. Particularly, stochastic first order methods which uses stochastic estimates $\tn f$ rather than the exact gradient $\nabla f$ not only reduces the cost of the computation, but also can provide differential privacy \cn. 

Due to persistent nature of the noise on the gradients, the performance of the stochastic SP methods \bcred{differs} from their deterministic counterparts and \bcred{depends} heavily on %. In particular, the convergence guarantees for deterministic first-order methods %may not imply 
%\sa{do not immediately translate to convergence guarantees} for the stochastic first-order methods; moreover, the iterates generated by the stochastic methods, \sa{being random variables, form a stochastic process. Thus,} 
\mg{the statistical properties of \sa{the limiting point/distribution generated as a solution} to the problem in \eqref{def: sapd-opt-prob}. In particular, addition of a momentum-averaging step has a typical affect to increase the stationary variance of the iterates in the context of stochastic momentum methods such as SAPD \cite{zhang2021robust} and in this context developing efficient variance-reduction strategies becomes a key for achieving better practical performance.}

\mg{
\textbf{Contributions.} In this paper, we consider the SAPD algorithm with constant (primal and dual) stepsize for solving \sa{SCSC} SP problems of the form %\eqref{def: SCSC-problem}
\sa{\eqref{def: sapd-opt-prob}}. Employing constant stepsize has at least two major benefits: (i) only one value needs to be tuned as opposed to \sa{$a,b$ and $c$ parameters needed to be tuned for decaying step size sequence of the form $a / (b+ck)$ for $k\geq 0$;} (ii) the ``bias term"\bcred{, which characterizes how fast \sa{the effects of initial conditions on} the iterates are forgotten,} decays exponentially (see Proposition \ref{prop: conv-of-SAPD}). 

Our contributions are as follows:
\begin{itemize}
    \item In Proposition \ref{prop: conv-of-SAPD}, we consider a parametrization of \sa{the primal stepsize $\tau$ and dual stepsize $\sigma$} in terms of the momentum parameter $\theta$ and obtain convergence guarantees for SAPD for that particular choice of parameters. \sa{For this specific parametrization of $\tau,\sigma$ in $\theta$, working directly with the expected distance square~(EDS) metric, rather than the more stronger expected gap metric as in~\cite{zhang2021robust}, we were able to provide 
    %(primal and dual stepsize and the momentum parameter),
    a sharper result for the EDS metric in terms of constants,} compared to those available for SAPD in %the literature from
    \cite{zhang2021robust}. \sa{Under this parametrization,} the corresponding linear convergence rate for the bias term is equal to the \sa{momentum} parameter $\theta$ \sa{as also shown in~\cite{zhang2021robust}}. For ill-conditioned problems we expect \sa{a} slower convergence \sa{for the bias as selecting small $\tau,\sigma>0$ requires $\theta \in (0,1)$ chosen close to $1$.}
    \item Under some assumptions on the gradient noise structure, we show that SAPD iterates admit an invariant distribution (Theorem \ref{thm: inv-meas-exists}). Since SAPD iterates result in a Markov chain that is \emph{non-reversible}, standard tools for reversible Markov Chains (such as those arising in the study of stochastic gradient descent methods \cite{bridging-the-gap}) are not directly applicable. We achieve this result by showing that so-called ``minorization and drift conditions" hold for the Markov chain corresponding to the SAPD iterates.
    \item In Lemma \ref{lem: finite-moment}, we characterize the second and fourth moments of the stationary distribution in terms of its dependency to the momentum parameter $\theta$. Building on this lemma, in Theorem~\ref{thm: expansion-at-inv-meas-mean}, we show that the expected iterates contain a bias that is proportional to $\mathcal{O}(1-\theta)$ as $\theta \to 1$. Motivated by this result, \sa{based on Richardson-Romberg extrapolation type arguments,} we propose a variance-reduction scheme: \sa{running SAPD %iterates are 
    twice independently with different parameters $\theta_1$ and $\theta_2$, one can remove the bias term proportional to $\cO(1-\theta)$ by considering a linear combination of the two iterate sequences corresponding to two appropriately chosen parameters $\theta_1$ and $\theta_2$}. We call this method variance-reduced SAPD (VR-SAPD). Although it is known that Richardson extrapolation can be very efficient for optimization algorithms such as stochastic gradient descent \cite{bridging-the-gap} and Frank-Wolfe methods \cite{bach-richardson}, to our knowledge, our paper provides the first application of this technique to the accelerated stochastic \sa{primal-dual algorithms for saddle-point problems}. There are also variance-reduction techniques for finite-sum problems where the objective is in the form of an average of finitely many component functions, e.g., \cite{palaniappan2016stochastic,chavdarova2019reducing,alacaoglu2021stochastic}; however, these techniques are not available to our setting as our objective is more general and we do not assume that it has a finite-sum structure.
    \item In Theorem \ref{thm: av-seq-conv}, we characterize the gap between \sa{the expected} ergodic average of SAPD iterates and \sa{the expectation of SAPD iterates in the limit} as the number of iterations $k$ grows. %The result
    \sa{We show} that this gap is of the order $\mathcal{O}(1/k)$ and is vanishing asymptotically; therefore, it implies that %similar 
    \sa{the same variance-reduction mechanism} can be applied to the ergodic averages of the SAPD iterates as well.
    \item We showcase the efficiency of our proposed algorithm VR-SAPD on distributionally robust logistic regression~\sa{(DRLR)} problems on three datasets where we compare VR-SAPD with SAPD \cite{zhang2021robust}, S-OGDA \cite{fallah_2020}, and Stochastic Mirror Prox (SMP) \cite{SMP} algorithms. %In this case, since 
    \sa{For the DRLR problem, we adopted $f_2$-divergence to define the uncertainty set around the uniform distribution; therefore, the problem domain is the Euclidean space, and in this case} SMP reduces to the stochastic gradient descent ascent (SGDA) method which is commonly used in machine learning practice, e.g., 
    %for instance 
    for training GANs \cite{kontonis2020convergence}. Our results show that VR-SAPD reduces the variance of the SAPD iterates considerably and \bcred{results} in a significant performance improvement.
\end{itemize}
}
%propose a variance-reduction %also becomes relevant for the stochastic methods. %There have been several work regarding the convergence and statistical properties of stochastic saddle point algorithms in the literature \cn. 



\textbf{Notations.} 
%For any $p\geq 1$, let $\mathcal{P}_{p}(\mathbb{R}^{2d})$ be the space consisting of all the Borel probability measures $\nu$ on $\mathbb{R}^{2d}$ with the finite $p$-th moment (based on the Euclidean norm). 
%For any two Borel probability measures $\nu_{1},\nu_{2}\in\mathcal{P}_{p}(\mathbb{R}^{2d})$, 
%orwe define the standard $p$-Wasserstein
%metric (see e.g. \cite{villani2008optimal}):
%$$\mathcal{W}_{p}(\nu_{1},\nu_{2}):=\left(\inf_{
%Z_{1}\sim\nu_{1},Z_{2}\sim\nu_{2}
%\sa{(Z_1,Z_2)\sim\Gamma(\nu_1,\nu_2)}}
%\mathbb{E}[\Vert Z_{1}-Z_{2}\Vert^{p}]\right)^{1/p},$$
%\todo[inline]{Bunu cikarabiliz.}
%where \sa{$\Gamma(\nu_1,\nu_2)$ denotes the set of joint probability distributions with marginals $\nu_1$ and $\nu_2$ on the first and second factors, respectively.}
%Let $S\in \mathbb{R}^{2d\times 2d}$ be a symmetric positive definite matrix. 
\sa{Let $\mathbb{R}_+$ is the set of positive real numbers.} For any vector $v \in \mathbb{R}^d$, $\Vert x \Vert$ \sa{denotes the Euclidean norm, %of the vector, 
and for any matrix $M\in\mathbb{R}^{d_x\times d_y}$, $\Vert M \Vert_2$ denotes the spectral norm, 
%of the matrix $M$, 
i.e., the largest singular value of $M$.}
Let $E$ and $F$ be two real vector spaces. \mg{We use $E\otimes F$ to denote the tensor product of $E$ and $F$}. \mg{The tensor product of two vectors $x\in E$ and $y\in F$ is denoted as \sa{$E\otimes F \ni x\otimes y =xy^\top$}}.  Similarly, $E^{\otimes k}$ is the k-th tensor power of $E$ and $x^{\otimes k}\in E^{\otimes k}$ is the  k-th tensor product of $x\in E$. \bcred{We use $\mathbb{N}$ for the set of non-negative integers, and $\mathbb{N}_+\triangleq\mathbb{N}\setminus \{0\}$.}
Let $n\in \mathbb{N}_{+}$, then $\bcred{\mathcal{C}^{n}(\mathbb{R}^d,\mathbb{R}^{m})}$ is the set of n-times continuously differentiable functions from $\mathbb{R}^{d} \rightarrow \mathbb{R}^{m}$. Let $f \in \mathcal{C}^{n}(\mathbb{R}^{d},\mathbb{R}^{m})$, \bcred{$D^{n}f$} is
% the notations $D^{n}F$ or $F^{(n)}$ denote 
the $n$-th differential of $f$. \bcred{If $f\in\mathcal{C}^{n}(\mathbb{R}^{d},\mathbb{R})$, then  $\bcred{\nabla}^{(n)}f(z)$ denotes the tensor of order $n$ at the point $z\in\mathbb{R}^{d}$ \mg{arising in the Taylor expansion of $f$}.} For any vector $z\in\mathbb{R}^{d}$ and any matrix $M\in\mathbb{R}^{d\times d}$, we define $[\bcred{\nabla}^{(3)}f(\bcred{z})M]_{\ell}=\sum_{i=1}^{d}\sum_{j=1}^dM_{i,j} \frac{\partial^{3}f}{\partial \bcred{z}_{i}\partial \bcred{z}_j\partial \bcred{z}_\ell}(\bcred{z})$.
%\nsa{Here we should use $\partial$ rather than $\delta$, right?} 
\bcred{For any matrices $M, N\in \mathbb{R}^{d\times d}$ $M\otimes N$ is defined as the endomorphism of $\mathbb{R}^{d\times d}$ such that $M\otimes N: P \rightarrow \bcred{MPN^\top}$.}
%We denote the Kronecker product by $\otimes$. 
Lastly, $(x_*,y_*)$ is the \sa{unique} solution of the \sa{SP} problem \sa{in} \eqref{def: sapd-opt-prob} and 
%the notations 
$\nabla^{(2)}f_*$ and $\nabla^{(3)}f_*$ are used for $\nabla^{(2)}f(x_*,y_*)$ and $\nabla^{(3)}f(x_*,y_*)$, respectively, for simplicity.
% \begin{algorithm}
% \caption{SAPD}\label{alg: sapd}
% \textbf{Input:} $K\in \mathbb{N}, \{\tau,\sigma,\theta\}, x_0\in\mRx, y_0 \in \mRy$ \\
% Set $x_{-1}\gets x_0$ and $y_{-1}\gets y_0$\\
% \For{$k=1,..,K$}{
% $\tilde{q}_k\gets\tn_y f(x_k,y_{k})-\tn_y f(x_{k-1},y_{k-1})$\\
% $\tilde{s}_k\gets \tn_y f(x_k,y_k)+\theta \tilde{q}_k$\\
% $y_{k+1}\gets \mathbf{prox}_{\sigma g}(y_k+\sigma \tilde{s}_k)$\\
% $x_{k+1}\gets \mathbf{prox}_{\tau f}(x_k-\tau \tn_xf(x_k,y_{k+1}))$
% }
% \end{algorithm}
\section{Preliminaries and Background}
\mg{\paragraph{SAPD Algorithm.} Recently, %been proposed by
Zhang \emph{et al.} \cite{zhang2021robust} have proposed the (SAPD) algorithm} to solve \sa{SCSC SP problems of the form} \eqref{def: sapd-opt-prob}. \sa{SAPD updates are given as follows:} 
%consisting of the iterates
\begin{subequations}\label{alg: sapd}
\begin{align}
\tilde{q}_k&= (1+\theta)\tn_y f(x_k,y_k)-\theta \tn_y f(x_{k-1},y_{k-1}),\\
%\tilde{s}_k
 \sa{y_{k+1}}
&= y_k+\sigma \tilde{q}_k,\\
x_{k+1}&= x_k-\tau \tn_xf(x_k, \sa{y_{k+1}}). %\tilde{s}_k)
\end{align}
\end{subequations}
Basically, SAPD admits three \sa{positive} parameters $(\tau,\sigma,\theta)$ where $\tau$ is the primal stepsize, $\sigma$ is the dual stepsize, and $\theta$ is the momentum parameter. %primal and dual stepsizes 
%In the same paper, the authors studied the convergence and robustness of SAPD algorithm.
In our work, we are particularly interested in \sa{designing a method for the SP problem in \eqref{def: sapd-opt-prob}}
 %developing saddle point algorithms  
 that would improve the variance of \sa{the SAPD iterate sequence $\{(x_k,y_k)\}_{k\geq 0}$. We call our method \emph{Variance Reduced SAPD}~\mg{(VR-SAPD)}.} \mg{For analysis purposes, we 
 %start with introducing 
 \sa{first state} our assumptions on $f$ and \sa{$\tilde\grad f$}.}%on the gradient noise.
%\sa{satisfying} Assumption \ref{assump: obj-fun-prop}.
\begin{assumption}\label{assump: obj-fun-prop} \sa{We assume $f\in\cC^4$, i.e., four times continuously differentiable} \bc{with uniformly bounded \sa{$3$-rd and $4$-th order} derivatives}. For any $\hat{y}\in \mRy$, \sa{$f(\cdot,\hat{y})$} is \sa{$L_{xx}$-smooth} and 
$\mu_x$-strongly convex for some \sa{$L_{xx},\mu_x>0$}. %with respect to $x$ 
Furthermore, for any $\hat{x}\in\mRx$, %the function 
\sa{$f(\hat{x},\cdot)$} is %\sa{$L_{yy}$-smooth} and 
$\mu_y$-strongly concave, \sa{and there exist constants $L_{yx},L_{yy}> 0$ such that
\begin{align*}
% &\Vert \nabla_x f(x,y)- \nabla_x f(\hat{x},\hat{y})\Vert \leq L_{xy}\Vert y-\hat{y}\Vert+ L_{xx}\Vert x-\hat{x}\Vert,\\
&\Vert \nabla_y f(x,y) - \nabla f_y(\hat{x},\hat{y})\Vert \leq L_{yx}\Vert x-\hat{x}\Vert + L_{yy}\Vert y-\hat{y}\Vert,
\end{align*}
for all $x,\hat{x} \in \mRx$ and $y,\hat{y}\in \mRy$.}
%with respect to $y$. 
% Furthermore, \sa{there exists $L_{yx}>0$ such that} the Hessian of $f$, \sa{$\grad^{(2)}f$,} satisfies
% \begin{align}\label{cond: Hessian_bounds}
%     \Vert \nabla^{\sa{(2)}}_{yx} f(x,y) \Vert_2 \leq L_{yx}, \quad \sa{\forall~x\in\mRx,~y\in\mRy}.
% \end{align}
\end{assumption}
%\nsa{We should give the definition of $L_{yx}$ using the first-order argument and remove the assumption on the Hessian.}
% \begin{remark}\label{remark: gradient-props} 
% % \sa{Since $f\in\cC^4$, \eqref{cond: Hessian_bounds} implies that $L_{xy} \triangleq L_{yx}$ satisfies $\Vert \nabla^{\sa{(2)}}_{xy} f(x,y)\Vert_2 \leq L_{xy}$ for all $x$ and $y$.} 
% A consequence of %the inequalities \eqref{cond: Hessian_bounds} in 
% \sa{Assumption \ref{assump: obj-fun-prop} is that 
% %the gradient with respect to $x$, i.e. $\nabla_x f(x,y)$, 
% $\grad_x f$ and $\grad_y f$ are Lipschitz:} %$L_{xy}$-Lipschitz, that is
% \begin{align*}
% % &\Vert \nabla_x f(x,y)- \nabla_x f(\hat{x},\hat{y})\Vert \leq L_{xy}\Vert y-\hat{y}\Vert+ L_{xx}\Vert x-\hat{x}\Vert,\\
% &\Vert \nabla_y f(x,y) - \nabla f_y(\hat{x},\hat{y})\Vert \leq L_{yx}\Vert x-\hat{x}\Vert + L_{yy}\Vert y-\hat{y}\Vert,
% \end{align*}
% for all $x,\hat{x} \in \mRx$ and $y,\hat{y}\in \mRy$.
% \end{remark}
\sa{We also make the following standard assumption on $\tilde\grad f$, which says that we 
have access to unbiased stochastic estimates of the gradients.}

\begin{assumption}\label{assump: noise-properties} 
%At an iterate $(x,y)$, %we assume 
\sa{Let $\{x_k,y_k\}$ be the SAPD iterate sequence. For all $k\geq 0$,
we have access to $\tn_y f (x_k,y_k,\sa{\zeta_k^y})$ and $\tn_x f(x_k,y_{k+1},\sa{\zeta_k^x})$ which are unbiased estimates of $\nabla_y f(x_k,y_k)$ and $\nabla_x f(x_k,y_{k+1})$, respectively;\footnote{\sa{$\zeta_k^y$ and $\zeta_k^x$ are determining the noise structure, and for simplicity of the notation we suppress them and use $\tilde\grad_y f(x_k,y_k)$ and $\tilde\grad_x f(x_k,y_{k+1})$ instead.}} i.e.,
\begin{align*}
    &\mathbb{E}[\tn_y f(x_k,y_k,\zeta_k^y)| x_k,y_k]=\nabla_y f(x_k,y_k),\\
    &\mathbb{E}[\tn_x f(x_k,y_{k+1},\zeta_k^x) | x_k,y_{k+1}]=\nabla_x f(x_k,y_{k+1}),
\end{align*}
such that
%for two random variables $\zeta^x$ and $\zeta^y$ that are independent from each other. 
%Moreover, there exist $\delta_{(p)}>0$ such that for all $k\geq 0$, given $(x_k,y_k,y_{k+1})$, the stochastic gradients $\tn_x f(x_{k},y_{k+1}; \eta_k^x)$, $\tn_y f(x_k,y_k; \eta_k^y)$, and  
the $\{\zeta_k^x\}_k$ and $\{\zeta_k^y\}$ are independent sequences and also independent from each other. Furthermore, for $p\in\{2,3,4\}$, 
%both estimates have bounded $p$-th moments 
there exists $\delta_{(p)}>0$ such that
{\small
\begin{subequations}
\label{ineq: noise-var}
\begin{align}
&\mathbb{E}[\Vert \tn_y f(x_k,y_k,\zeta^y_k)-\nabla\bcred{y} f(x_k,y_k)\Vert^{p}] \leq \sa{\delta_{(p)}^p},\\
&\mathbb{E}[\Vert \tn_x f(x_k,y_{k+1},\zeta^x_k)-\nabla_{\bcred{x}} f(x_k,y_{k+1})\Vert^{p}] \leq \sa{\delta_{(p)}^p}.
\end{align}
\end{subequations}}%
}%
\bc{\sa{We also assume that both noise, i.e.,} $\tn_xf-\nabla_xf$ and $\tn_yf-\nabla_yf$, are stationary, and \bcred{independent from the \mg{past}.}} %$\{x_k,y_k\}_{k\in\mathbb{N}}$}, and measurable with respect to the sigma-algebra generated by the iterates $\{x_k,y_k\}_{k\in\mathbb{N}}$.
\end{assumption}
\mg{We note that $f$ being twice continuously differentiable and existence of second moments for the gradient noise would be sufficient to obtain convergence guarantees \sa{in $L^2$ for the accumulation of SAPD sequence $\{x_k,y_k\}$ in the vicinity of the unique saddle point--see Theorem~\ref{thm:complexity} below}; however, \sa{in this paper}, we require further smoothness up to fourth order to be able to obtain stronger convergence guarantees for the fourth moments which is then used in our variance reduction mechanism (see~Lemma~\ref{lem: finite-moment} and Theorem \ref{thm: expansion-at-inv-meas-mean}).}
 %generated by stochastic accelerated primal dual algorithm (SAPD).
%We make the following assumption on the noise at the gradient estimates $\tn f$ that are used at Algorithm \ref{alg: sapd}.
%\nsa{I suggest we use $\delta_{(p)}^p$ notation in the above assumption. We used $\tau$ for the primal step size. And in case the reader refers to SAPD paper, $\sigma$ is adopted for the dual step size and $\delta^2$ is the noise variance.}

\mg{The next result, which is a direct consequence of Theorems 2.6 and 2.9 in~\cite{zhang2021robust}, summarizes the known iteration complexity results for SAPD with \sa{constant primal and %constant
dual stepsizes.}}
\begin{theorem}[\cite{zhang2021robust}]
\label{thm:complexity}
\sa{Consider the problem in~\eqref{def: sapd-opt-prob}. Under Assumptions~\ref{assump: obj-fun-prop} and~\ref{assump: noise-properties} for $p=2$, given any $\epsilon>0$, there exists $\hat{\theta}_\epsilon\in(0,1)$ such that the SAPD iterate sequence $\{x_k,y_k\}$ generated using
 $\tau=\frac{1-\theta}{\mu_x\theta}$ and $\sigma=\frac{1-\theta}{\mu_y\theta}$
for any $\theta\in \sa{[}\hat{\theta}_\epsilon, 1)$ satisfies 
{\small
$$\mathbb{E}\left[\max\{\sup_{x,y}\{f(\bar{x}_N,y)-f(x,\bar{y}_N)\},~\norm{z_N-z^*}^2\}\right]\leq \epsilon,$$} 
for all $N\geq N_\epsilon\in\bcred{\mathbb{N}_+}$ such that
{\scriptsize
\begin{align*}
    N_\epsilon=\tilde\cO\left(\Big(\frac{L_{xx}}{\mu_x}+\frac{L_{yx}}{\sqrt{\mu_x\mu_y}}+\frac{L_{yy}}{\mu_y}\Big)\log\Big(\frac{1}{\epsilon}\Big)+\Big(\frac{1}{\mu_x}+\frac{1}{\mu_y}\Big)\frac{\delta_{(2)}^2}{\epsilon}\right).
\end{align*}}}%
\end{theorem}
%\begin{proof}
%\sa{This result immediately follows from Theorems 2.6 and 2.9 in~\cite{zhang2021robust}.}
%\end{proof}
\sa{Here $\tilde\cO(\cdot)$ notation hides $\log(1/\epsilon)$ factor for the variance term, which can be removed adopting a restart approach proposed in~\cite{fallah_2020}. Let $$\kappa_x\triangleq L_{xx}/\mu_x, \quad \kappa_y\triangleq L_{yy}/\mu_y, \quad \kappa_{yx} \triangleq L_{yx}/\sqrt{\mu_x\mu_y},$$ and define $\kappa\triangleq \max\{\kappa_x,\kappa_y,\kappa_{yx}\}$. In the above result, the first part $\cO(\kappa\log{1/\epsilon})$ is related to the bias term; it is essential to emphasize that the bias term for SGDA using constant step size is $\cO(\kappa^2\log{1/\epsilon})$. Thus, SAPD %significantly 
accelerates the convergence of the bias term compared to the popular alternative SGDA.}

\paragraph{Dynamical system representation of SAPD.} %\mg{If we introduce the following vectors that concatenate the iterates and the gradients,}
\sa{Through defining the following concatenations,}
\begin{align}
z_k\triangleq\begin{bmatrix} 
x_k\\
y_k
\end{bmatrix},\;
\xi_k\triangleq \begin{bmatrix} 
z_k\\
z_{k-1}\\
\end{bmatrix}, 
\tPhi_k\triangleq\begin{bmatrix} \tn_x f(x_{k}, %\tilde{s}_k
\sa{y_{k+1}})\\
\tn_y f(x_k,y_k)\\
\tn_y f(x_{k-1},y_{k-1})
\end{bmatrix},
\end{align}
\sa{the SAPD recursion in \eqref{alg: sapd}} can be rewritten as %the dynamical system
\begin{equation}\label{alg: sapd-dyn-sys}
\xi_{k+1}= M \xi_k + N \tPhi_k,
\end{equation}
with the associated matrices 
{\small
\begin{align*}
M=\begin{bmatrix} 
I_d & 0_d \\
I_d & 0_d
\end{bmatrix},\  
N= \begin{bmatrix}
-\tau I_{d_x} & 0_{d_x\times d_y} & 0_{d_x\times d_y}\\
0_{d_y\times d_x} &  \sigma(1+\theta)I_{d_y} & -\theta \sigma I_{d_y}\\ 
0_{d_x\times d_x} &  0_{d_x\times d_y} & 0_{d_x\times d_y}\\
0_{d_y} & 0_{d_y} & 0_{d_y} 
\end{bmatrix},
\end{align*}}%
with $d\triangleq d_x+d_y$. In some places, we will also use the notation $\xitdt_k$ interchangeably with $\xi_k$ to emphasize the iterates' dependency on the parameters of the algorithm. 

\paragraph{SAPD iterates as a Markov Chain.} We notice that under Assumption~\ref{assump: noise-properties}, the iterates $\{\xitdt_k\}_{k\in\mathbb{N}}$ define a \sa{time-homogeneous} Markov chain. Let $\mcRtdt$ be the Markov kernel of iterates $\{ \xitdt_k\}_{k\in\mathbb{N}}$ on $(\mathbb{R}^{2d},\mathcal{B}(\mathbb{R}^{2d}))$, \mg{where $\mathcal{B}(\mathbb{R}^{2d})$ is the sigma-algebra generated by the Borel sets in $\mathbb{R}^{2d}$}, i.e., %for all $k\in\mathbb{N}^{+}$, %\mg{for all Borel sets} $A\in\mathbb{R}^{2d}$ and
\sa{for all $A\in\mathcal{B}(\mathbb{R}^{2d})$ and $k\geq 0$,} %\mg{$\xi_k\in\mathbb{R}^{2d}$}, 
$$\mcRtdt(\xi_k,A)=\mathbb{P}\{ \xi_{k+1}\in A | \xi_k \},\quad\forall \xi_k\in\mathbb{R}^{2d},$$ 
almost surely, \mg{the map} \mg{$\xi\mapsto \mcRtdt(\xi,A)$} is Borel measurable, and $\mcRtdt(\xi_0, \cdot)$ is a probability measure on $(\mathbb{R}^{2d},\mathcal{B}(\mathbb{R}^{2d}))$ \sa{for any $\xi_0\in\mathbb{R}^{2d}$}. \sa{Then, for all $k\geq 1$, the Markov kernel associated with} $\mcRtdt_k$ of $\xi_k$ is recursively defined for any $\xi_0\in\mathbb{R}^{2d}$ and $A\in \mathcal{B}(\mathbb{R}^{2d})$ as 
$$
\mcRtdt_{k+1}(\xi_0, A) = \int_{\mathbb{R}^{\sa{2}d}}\mcRtdt_{k}(\xi_0, d\xi)\mcRtdt(\xi,A),
$$
where $\mcRtdt_1=\mcRtdt$. We also define %the probability measure
$\lambda \mcRtdt_k$ for any probability measure $\lambda$ on $(\mathbb{R}^{2d}, \mathcal{B}(\mathbb{R}^{2d}))$ by 
$$
\lambda \mcRtdt_k(A) \triangleq\int_{\mathbb{R}^{\sa{2}d}}\lambda(d\xi)\mcRtdt_k(\xi,A),\  \forall~A \in \mathcal{B}(\mathbb{R}^{2d}).
$$
%Notice that 
The above definition implies that for \mg{any} probability measure $\lambda$ on $\mathcal{B}(\mathbb{R}^{2d})$ and $k\in \mathbb{N}_{+}$, $\lambda \mcRtdt_k$  is the distribution of $\xitdt_k$ %started 
\sa{initialized} from \sa{$\xi_0\sim\lambda$, i.e., $\xi_0$ %$\xi_0^{\top}=[z_0^\top, z_{0}^{\top}]$ where $z_0$ is 
drawn from $\lambda$}. For any function $\Psi: \mathbb{R}^{2d}\rightarrow \mathbb{R}$ and $k\in\mathbb{N}_{+}$, the measurable function $\mcRtdt_k\Psi:\mathbb{R}^{2d}\rightarrow \mathbb{R}$
is defined as %follows for all $\xi_0\in\mathbb{R}^{2d}$,
$$
\mcRtdt_k\Psi (\xi_0)\triangleq\int_{\mathbb{R}^{\sa{2d}}}\Psi(\xi)\mcRtdt_k(\xi_0,d\xi),\quad\sa{\forall~\xi_0\in\mathbb{R}^{2d}}.
$$
For any measure $\lambda$ on $(\mathbb{R}^{2d},\mathcal{B}(\mathbb{R}^{2d}))$ and any measurable function $h:\mathbb{R}^{2d}\rightarrow \mathbb{R}$, we denote $\int_{\mathbb{R}^{\sa{2d}}}h(\xi)d\lambda(\xi)$ by $\lambda(h)$ (whenever exists) for simplicity. Notice that this notation implies the equality $\lambda(\mcRtdt_k h)= (\lambda \mcRtdt_k)(h)$ for any measure $\lambda$ on $\mathcal{B}(\mathbb{R}^{2d})$ and any measurable function $h:\mathbb{R}^{2d}\rightarrow \mathbb{R}$ and $k\in\mathbb{N}_{+}$. A distribution $\ptdt$ is called an \textit{invariant measure} for $\mcRtdt$ if \bcred{$\ptdt\mcRtdt=\ptdt$}and we say the Markov chain $\{ \xitdt_k\}_{k\in\mathbb{N}}$ is \textit{stationary} if it admits an invariant measure $\ptdt_*$, \sa{i.e., $\xitdt_0$} is distributed according to $\ptdt_*$ implies that the distribution of $\xitdt_k$ is also $\ptdt_*$ for all $k\in\mathbb{N}$. \bc{Depending on the context, we use the notation $\pi_{*}$ interchangeably with $\pi_{*}^{(\tau,\delta,\theta)}$ for simplicity. Similarly, \mg{when all the parameters of the SAPD algorithm are parametrized as function of $\theta$}, then we %set
\sa{adopt the notation} $\pi_*^{(\theta)} \triangleq\pi_*^{(\tau_{\theta},\sigma_{\theta},\theta)}$,} and \mg{similarly, 
% we %adapt 
% \sa{adopt} the notations
$\xi_k^{(\theta)}\triangleq \xi_k^{(\tau_{\theta},\sigma_{\theta},\theta)}$ and $\mcR^{(\theta)}\triangleq\mcR^{(\tau_\theta,\sigma_\theta,\theta)}$.%, and %$\pi_*^{(\theta)}\triangleq \pi_{*}^{(\tau_\theta,\sigma_{\theta},\theta)}$
}








==> [Arxiv] Variance Reduced SAPD-2/sections/numerical-experiments.tex <==
\section{Numerical Experiments}
In this section, we compare the performance of VR-SAPD with SAPD \cite{zhang2021robust}, S-OGDA \cite{fallah_2020}, and SMP \cite{SMP} on the $\ell_2$-regularized distributionally robust learning problem
\begin{equation}\label{def: DRO}
    \min_{x\in \mathcal{S}}\max_{y\in \mathcal{P}_r}\sa{f_{0}}(x,y)\triangleq \frac{\mu_x}{2}\Vert x \Vert^2 + \sum_{i=1}^{n}y_i \phi_i(x)\tag{DRO},
\end{equation}
where $\mathcal{S}\triangleq \{x \in\mathbb{R}^d : \Vert x \Vert^2 \leq \mathcal{D}_x \} $ for some diameter $\mathcal{D}_x>0$ and $\phi_i:\mathbb{R}^d\rightarrow \mathbb{R}$ \sa{is a convex loss function corresponding to the $i$-th data point for $i=1,\ldots,n$.} 
%strongly convex function with respect to $x$ and depends on the 
\mg{While \sa{for} the %standard 
\sa{classic} empirical risk minimization \sa{problem} 
%corresponds to the case when 
the weights are selected %uniformly with 
\sa{as} $y_i = 1/n$ for every $i=1,\ldots,n$, the robust formulation \sa{in}~\eqref{def: DRO} \sa{allows for $\{y_i\}_{i=1}^n$ to 
%belong to 
come from} an uncertainty set around the uniform weights
%The constraints on the parameters are given as and
$\mathcal{P}_r \triangleq \{ y \in \mathbb{R}_+^n : \mathbf{1}^\top y=1, \Vert y-\mathbf{1}/n \Vert^2 \leq \frac{r}{n^2} \}$  whose radius is controlled by the parameter $r$, where $\mathbf{1}$ is the vector %with all entries being 
\sa{of all ones} --see the experimental section in~\cite{zhang2021robust} for more details.}

\mg{The DRO formulation is %linear
\sa{affine} in the variable $y$; \sa{hence,} not strongly concave in $y$. However, in a similar spirit to Nesterov's smoothing technique \cite{Nesterov}, we can introduce a %standard 
dual regularizer to have a SCSC approximation to %the problem 
\eqref{def: DRO}}. \sa{This corresponds to approximating the original problem in the primal form that is non-smooth with a smooth primal optimization problem. Indeed, we will implement VR-SAPD algorithm on}
\begin{small}
\begin{equation} \label{def: SCSC-problem}
\min_{x\in \mathcal{S}} \max_{y\in \mathcal{P}_r} f(x,y) \triangleq \frac{\mu_x}{2}\Vert x \Vert^2 + \sum_{i=1}^{n}y_i \phi_i(x) - \frac{\mu_y}{2}\Vert y\Vert^2 \tag{\sa{Reg-DRO}},
\end{equation}
\end{small}%
where $\mu_y$ is chosen appropriately, \sa{i.e., $\mu_y=\Theta(\epsilon)$.} \bc{In particular, if we choose  $\mu_y=\frac{\epsilon}{2\mathcal{D}_y}$ where $\mathcal{D}_y\sa{\triangleq}\sup_{y\in \mathcal{P}_r}\Vert y\Vert^2=1$ \sa{for} \eqref{def: SCSC-problem} and find a solution $(\bar{x},\bar{y})$ satisfying $\mE[\sup_{(x,y)\in\mathcal{S}\times \mathcal{P}_r}\sa{\{}f(\bar{x},y)-f(x,\bar{y})\sa{\}}]<\frac{3\epsilon}{4}$, then it can be shown that $(\bar{x},\bar{y})$ also satisfies $\mE[\sup_{(x,y)\in\mathcal{S}\times \mathcal{P}_r}\sa{\{f_0}(\bar{x},y)-\sa{f_0}(x,\bar{y})\sa{\}}]<\epsilon$.}  %(as a function of the target accuracy $\varepsilon$ and apply the VR-SAPD algorithm. 
In the following, we consider the binary logistic loss function $\phi_i(x)=\log(1+\exp(-b_i a_i^\top x))$ calculated at \sa{the $i$-th} data point from $\{a_i,b_i\}_{i\in \{1,..,n\}}$, and we set $r=2\sqrt{n}$. Notice that the objective of \eqref{def: SCSC-problem} admits Lipschitz constants $L_{xy}=L_{yx}=\Vert A \Vert_2$, $L_{xx}=\max_{i=1,..,n}\{\frac{1}{4}\Vert a_i \Vert^2_2 \}$, and $L_{yy}=0$ where $A\in\mathbb{R}^{n\times d}$ is the data matrix with rows $\{a_i\}_{i=1}^{n}$ and columns $\{A_j\}_{j=1}^d$. 
%For satisfying the constraints, 
\sa{To stay feasible at each iteration, after performing $y_{k+1}$ and $x_{k+1}$ steps as in \eqref{alg: sapd}, we computed the \sa{Euclidean} projection onto} the constraint sets $\mathcal{S}$ and $\mathcal{P}_r$. \mg{In our theoretical results, for the simplicity of the presentation, we considered SAPD without projection steps. However, our convergence results to the stationary distribution extend in a straightforward manner when such projection steps are included.}\footnote{\mg{This is because the projection is a non-expansive operation \cite{bertsekas2015convex} which does not increase the distance to the solution and therefore the minorization and drift conditions will still hold for our distance-based Lyapunov function \eqref{def: lyap-func} after minor modifications to the proof of Theorem \ref{thm: inv-meas-exists}}.} 

%\nsa{Asagidaki plotlarda accuracy iyi durmuyor, orada relative error vermeyi konusmustuk eger $\norm{z^*}^2>1$ ise}
% Notice that the algorithm \eqref{alg: sapd} does not guarantee the constraints of \eqref{def: SCSC-problem}; however, this issue can be solved by introducing the updates at \eqref{alg: sapd}, 
% \begin{subequations}\label{alg: const-sapd}
% \begin{align}
%     y_{k+1}&= \underset{{y'\in \mathcal{P}_r}}{\text{argmin}}\{\frac{\sigma \mu_y}{2}\Vert y'\Vert^2+ \frac{1}{2}\Vert y_k+\sigma \tilde{q}_k-y'\Vert^2\}\\
%     x_{k+1}&= \underset{{x'\in \mathcal{S}}}{\text{argmin}}\{\frac{\tau\mu_x}{2}\Vert x' \Vert^2\nonumber\\ 
%     &\quad\quad\quad\quad+ \frac{1}{2}\Vert x_k-\tau \tn_xf(x_k,y_{k+1})-x'\Vert^2\}.
% \end{align}
% \end{subequations}

To illustrate our results from Section \ref{sec: var-red-sapd}, % that the mean of the averaging sequence $\tilde{\xi}_k^{(\theta)}$ generated by the SAPD algorithm \eqref{alg: sapd} to solve the problem \eqref{def: sapd-opt-prob} results in the performance bounds given in \eqref{eq: mean-av-seq}. Suppose 
we consider two sequences $\xi_k^{(\theta_1)}$ and $\xi_{k}^{(\theta_2)}$, \sa{both initialized with the same point $\xi_0$,} where %which are subject to same noise and started from same $\xi_0$.
\sa{such that} $\theta_2=2\theta_1-1$; and then consider the performance of the interpolated sequence $2\tilde{\xi}_{k}^{(\theta_1)}-\tilde{\xi}_{k}^{(\theta_2)}$. %satisfies the following condition in the limit, 
% \begin{equation*}
% \lim_{k\rightarrow \infty}\mE[ 2\tilde{\xi}_k^{(\theta_1)}-\tilde{\xi}_{k}^{(\theta_2)}] =\xi_*+\mathcal{O}((1-\theta)^{3/2}),
% \end{equation*}
% which improves the distance to global optimum by $\mathcal{O}\left(1-\theta\right)$.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/arcene_comparison.jpg}
    \caption{Comparison of S-OGDA, SMP, SAPD, and VR-SAPD on the Arcene data set in terms of the \bcred{relative} expected distance squared \bcred{$\mathbb{E}\|z_k - z_*\|^2/\Vert z_0-z_*\Vert^2$} as a performance metric.}
    \label{fig: arcene-fig}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/DryBean_comparison.jpg}
    \caption{Comparison of S-OGDA, SMP, SAPD, and VR-SAPD on the Dry Bean data set in terms of the relative expected distance squared $\mathbb{E}\|z_k - z_*\|^2/\Vert z_0-z_*\Vert^2$ as a performance metric.}
    \label{fig: drybean-fig}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/mnist_comparison.jpg}
    \caption{Comparison of S-OGDA, SMP, SAPD, and VR-SAPD on the MNIST data set in terms of the \bcred{relative} expected distance squared \bcred{$\mathbb{E}\|z_k - z_*\|^2/\Vert z_0-z_*\Vert^2$} as a performance metric.}
    \label{fig: mnist-fig}
\end{figure}%

We consider the algorithms VR-SAPD %(with the updates \eqref{alg: const-sapd})
, SAPD, S-OGDA, and SMP on three datasets:
\begin{enumerate}
    \item Dry Bean dataset \cite{DryBean} with $(n,d)=(9528, 16)$;
    \item Arcene dataset \cite{Arcene} with $(n,d)=(97,10000)$;
    \item MNIST dataset \cite{lecun1998gradient2} for hand-written digit classification with \bcred{$(n,d)=(1000,400)$}.
\end{enumerate}
Throughout the experiments, we set the regularization parameter $\mu_x$ through cross-validation and defined the parameters $(\tau_{\theta}, \sigma_\theta)$ of both VR-SAPD and SAPD as given in Proposition \ref{prop: conv-of-SAPD}, tuning the parameter as $\theta=0.95$. The gradients are estimated from mini-batches of data sampled at random with replacement where we have a batch size of $10$. At Dry Beans, we set $\mu_x=0.01$, $\mu_y=10$. %, and mini-batch size is $10$. 
We normalize each feature column $A_j\in\mathbb{R}^n$ using $A_j= \frac{A_j-\min(A_j)}{\max(A_j)-\min(A_j)}$ where max and min are taken over the elements of $A_j$. For the Arcene data set, we set $\mu_x=0.02$ and $\mu_y=10$ and normalize the data as $A\leftarrow A/\min\{\sqrt{d},\sqrt{n}\}$. Lastly, we set $\mu_x=0.1$, $\mu_y=10$ and mini-batch size $10$ for MNIST. We set $b_i=1$ if the i-th data point is number four and set $b_i=-1$, otherwise.

We generated two sequences $\{z^{(\theta_1)}_k\}_{k\in \mathbb{N}}$ and $\{z^{(\theta_2)}_k\}_{k\in\mathbb{N}}$ with $\theta_1=\theta$ and $\theta_2=2\theta-1$. For VR-SAPD, we considered the extrapolated sequence $z_k=2z_k^{(\theta_1)}-z_k^{(\theta_2)}$. The step-size of S-OGDA and SMP are taken as $\frac{1}{L}$ and $\frac{1}{\sqrt{L}}$, respectively, where $L=\max\{L_{xx}+\mu_x, \mu_y, L_{xy}, L_{yx}\}$.
\bcred{We generated 50 random sample paths to compute the mean and the variance of $\{\Vert z_k-z_*\Vert^2\}_{k=1}^K$ generated by the algorithms, \sa{each running for $K=1000$ iterations},}
% In Figures \ref{fig: arcene-fig} and \ref{fig: drybean-fig}, we plotted the mean and the optimization error $\{\Vert z_k-z_*\Vert^2\}_{k\in\mathbb{N}}$ using the 50 random sample paths 
where we %compute 
\sa{closely approximate} $z_*$ by running the deterministic APD algorithm~\cite{hamedani2021primal} until the change the loss function is below $\%0.01$. \mg{Our results for each dataset are summarized in Figures \ref{fig: arcene-fig}, \ref{fig: drybean-fig} and \ref{fig: mnist-fig} where we compared the methods in terms of the expected \bcred{relative} \sa{change in the} distance squared, \sa{i.e.,} $\mathbb{E}[\bcred{\frac{\|z_k - z_*\|^2}{\Vert z_0-z_*\Vert^2}}]$, as a performance metric \sa{--all the algorithms are initialized from %where the initialization is set to be 
$x_0= 2~\mathbf{1}_{d_x}$ and $y_0=1/d_{y}\mathbf{1}_{d_y}$.} 
%for vector of ones $\mathbf{1}_{d} \in\mathbb{R}^{d}$. 
For each method, we also display the standard deviation \sa{as the shaded region around the average of 50 sample paths.} Our results show that our variance reduction techniques result in a smaller asymptotic variance for the SAPD iterates as intended. We also see that VR-SAPD iterates admit a smaller variance in general compared to SAPD and improves upon the other methods SMP and S-OGDA. These results showcase the benefits of our variance reduction techniques.}

\section{Conclusion}
\mg{Under some assumptions, we showed that with constant stepsize, the distribution of the SAPD iterates admit a stationary distribution and characterized its dependency to the SAPD parameters. Based on these results, we introduced a variance-reduced stochastic accelerated primal-dual method (VR-SAPD), %Our methods are 
\sa{which is} based on Richardson-Romberg extrapolation. We also illustrated the efficiency and benefits of \sa{our %approach 
accelerated variance-reduced method} on robust training of logistic regression models.} %as an accelerated variance-reduced method.


\section{Acknowledgements}
This work was funded by the grants ONR N00014-21-1-2244, \sa{ONR N00014-21-1-2271}, NSF CCF-1814888 and NSF DMS-2053485. \bcred{We thank Xuan Zhang for providing \sa{us with the %initial
MATLAB implementations of SAPD, S-OGDA and SMP for our} numerical experiments.}


==> [Arxiv] Variance Reduced SAPD-2/sections/stochastic-acc-prim-dual.tex <==
\section{Variance Reduced SAPD}\label{sec: var-red-sapd}
\mg{%By the strong convexity/concavity of $f$, the problem 
\sa{Since $f$ is SCSC, the SP problem in} \eqref{def: sapd-opt-prob} admits a unique saddle point $z_* = (x_*, y_*)$. In the following result, \sa{we obtain convergence guarantees for %the squared distance of 
the SAPD iterates $(x_k, y_k)$ to the saddle-point %in expectation
in $L^2$.}
%, i.e., convergence in the 2-nd mean
%\todo{Burasi 2-nd moment olabilir mi?}
%\mg{in terms of the second moment of the distance to the saddle-point}. %Previously,
\sa{Recently,} convergence results for very general choice of SAPD parameters %were
\sa{are} given in \cite{zhang2021robust}. Our result considers a specific choice of parameters, \sa{for which} we can prove the existence of an invariant distribution for the iterates.}  
%\mg{For this specific choice of parameters (primal and dual stepsize and the momentum parameter), this is a sharper result compared to those available for SAPD in the literature from \cite{zhang2021robust}}.
\sa{For this specific choice of $\tau,\sigma$ in $\theta$, 
%working directly with the expected distance square~(EDS) metric, rather than the more stronger expected gap metric as in~\cite{zhang2021robust},
we were able to provide 
    %(primal and dual stepsize and the momentum parameter),
    a sharper result for the expected distance square metric in terms of constants,} compared to those available for SAPD in \cite{zhang2021robust}. 
% \sa{In our parameter selection}, the primal and dual step sizes, \sa{$\tau,\sigma>0$}, are parameterized by the momentum parameter $\theta$ and adapts and refines the convergence rate and asymptotic variance given in \cite{zhang2021robust} for this particular choice of parameters.


\begin{proposition}\label{prop: conv-of-SAPD}
Let the parameters $(\tau,\delta,\theta)$ of SAPD algorithm \eqref{alg: sapd} be chosen as, 
\begin{align}
\label{eq:SAPD-parameters}
    \tau_\theta\sa{\triangleq}\frac{1-\theta}{\mu_x \theta},\quad \sigma_\theta\sa{\triangleq}\frac{1-\theta}{\mu_y \theta},\; \sa{\theta \in [\hat{\theta}, 1),}
\end{align}
where $\hat{\theta}\triangleq\max\{\hat{\theta}_1,\hat{\theta}_2\} \in (0,1)$ and
%$\bar{\theta}_1$ and $\hat{\theta}_2$ are defined by 
%\notemg{Here, need to relate $\theta$ to $\bar\theta$? sorry i think i accidentally messed up what Bugra wrote earlier here.}
\begin{align*}
    %  \bar{\theta}_1&:= \frac{4L_{yx}^2+\mu_yL_{xx}}{4L_{yx}^2+\mu_yL_{xx}+\mu_x\mu_y}\\
    \hat\theta_1\triangleq \sa{\frac{1}{1+(\kappa_x+4\kappa_{yx}^2)^{-1}}<1}, \quad\quad\quad
    %  \bar{\theta}_2&:= \sqrt{\left(\frac{4L_{yy}^2}{\mu_y^2} +\frac{1}{2}\right)^2 + \frac{8L_{yy}^2}{\mu_y^2}}-\frac{4L_{yy}^2}{\mu_y^2}-\frac{1}{2}
    \hat\theta_2\triangleq\sa{\frac{2}{{\sqrt{(1+\tfrac{1}{8\kappa_y^2})^2+\frac{1}{2\kappa_y^2}}+1+\tfrac{1}{8\kappa_y^2}}}<1},
    % \sa{\sqrt{(4\kappa_y^2+\tfrac{1}{2})^2+8\kappa_y^2}-(4\kappa_y^2+\tfrac{1}{2})}
\end{align*}
where \sa{$\kappa_x=L_{xx}/\mu_x$, $\kappa_y=L_{yy}/\mu_y$ and $\kappa_{yx}=L_{yx}/\sqrt{\mu_x\mu_y}$,} the iterates $\{z_k\}_{k\in \mathbb{N}_{+}}$ satisfies, 
% \begin{equation}\label{cond: SAPD-convergence-result} 
% \mathbb{E}[\Vert z_k-z_*\Vert^2]\leq \mg{C_1} \theta^{k} \Vert z_0-z_*\Vert^2 + \frac{\theta (1-\theta^k)}{1-\theta}\Xi_{\theta}\delta_{(2)}^2,
% \end{equation}
\begin{align} 
\mathbb{E}\Big[{\mu_x}\Vert x_k-x_*\Vert^2 + \frac{\mu_y(1+\theta)}{2}\Vert y_k-y_*\Vert^2\Big]  \leq \theta^{k} \bcred{\Delta_0} + (1-\theta^k)\tilde{\Xi}_\theta \delta_{(2)}^2, \label{cond: SAPD-convergence-result}
\end{align}
where $z_*^\top=[x_*^\top,y_*^\top]$, $\Delta_0\triangleq{\mu_x}\Vert x_0-x_*\Vert^2 + {\mu_y}\Vert y_0 - y_*\Vert^2$, %\todo{Burada $\Delta_\theta$'ya ihtiyac yok degil mi direk $\Delta_0$ kullanabilirz aslinda. Appendix'te $\Delta$'yi kullaniyoruz. Burada baska bir notation kullanmamiz gerekir mi yoksa confusion olursturmaz mi?}
\begin{align*} 
\tilde\Xi_{\theta}\triangleq \frac{1-\theta}{\theta}\left(\frac{2}{\mu_x}+\frac{4}{\mu_y}\Big((1+\theta)^2+\theta^2\Big)\right).
\end{align*}
% \begin{align*} 
% \tilde\Xi_{\theta}:= \left(\frac{1-\theta}{\mu_{x}}\right)\Xi_{\theta}^x+ \frac{1-\theta}{\mu_y}\Xi_\theta^y+\frac{1}{2\eta_x}+\frac{1+2\theta}{\eta_y}\\
% \Xi_\theta^x&=1+\frac{\theta (1-\theta^2)L_{yx}}{2\mu_y}\\
% \Xi_{\theta}^{y}&= \left(1+2\theta + \theta^2\right)(1+2\theta)\\ 
% &\;+\left(\frac{\theta(1-\theta^2)L_{yy}}{\mu_y} +\frac{\theta (1-\theta)^2 (1+\theta)L_{yx}L_{xy}}{\mu_x\mu_y}\right)(1+2\theta)\\ 
% &\;+\frac{\theta(1-\theta^2)L_{yx}}{2\mu_x}
% \end{align*}

%\todo{there should be some cond. on $\eta_x, \eta_y >0$ for the result to hold; currently our bound is decreasing }
%\notemg{define what is $\eta_x, \eta_y$, making sure all the variables are well-defined}
\end{proposition}
%\nsa{We should give $C$ explicitly at least in the appendix.}
\mg{We are going to show that the invariant measure exists for the given choice of parameters in Proposition \ref{prop: conv-of-SAPD}. One %difficulty 
\sa{complication is that the Markov Chain corresponding to SAPD iterates becomes non-reversible due to the momentum term;} this can also be seen from the fact that the matrices $M$ and $N$ in the representation \eqref{alg: sapd-dyn-sys} are non-symmetric. Consequently, standard tools for showing the existence of a stationary measure for reversible Markov chains are not applicable to our setting. However, the results 
%of Hairer and Mattingly 
in~\cite{hairer2011yet} do not require reversibility and are applicable to our setting. More specifically, \cite{hairer2011yet} shows the existence of a stationary  distribution for a Markov Chain provided that \sa{the} so-called ``minorization and drift" conditions hold with certain parameters (see the appendix for the details). In the following, we introduce an assumption on the gradient noise which says that the gradient noise admits a continuous density. This assumption allows us to show that the ``minorization condition" holds.}

\begin{assumption}\label{assump-cont-density} The gradient noise admits a continuous density, %i.e. probability density of $z_{k+1}$ conditioned on $\xi_{k}$ is continuous,
\sa{i.e., $p$ defined such that $p(\xi, z) dz\triangleq\mathbb{P}( z_{k+1} \in dz | \xi_{k}=\xi)$ is continuous in $(\xi,z)$.} %both $\xi$ and $z$.
\end{assumption}
\mg{The \bcred{minorization} condition from \cite{hairer2011yet} for the transition kernel $\mathcal{R}$ of SAPD iterations \sa{shown in~\eqref{alg: sapd}} requires the existence of a Lyapunov function $\mathcal{V}:\mathbb{R}^{2d}\rightarrow \bcred{[0,\infty)}$ and constants $K\geq 0$ and $\zeta \in (0,1)$ such that 
\begin{equation}
(\bcred{\mcRtdt}\mathcal{V})(\sa{\xi}) \leq \zeta \mathcal{V}(\sa{\xi}) + K,
\label{cond-major-main-text}
\end{equation}
for every $\sa{\xi} \in \mathbb{R}^{2d}$. For this purpose, we devised the following Lyapunov function %Since momentum-based averaging can cause a non-monotonic behavior in the distance of the iterate sequence $z_k$ to $z_*$ \cite{zhang2021robust}, 
}
%\nsa{Is above equality a definition, i.e., is it the definition of $p$? We don't have $k$ dependence because of Markov chain being time homogeneous? So $p$ is related to Markov kernel...}
%\nsa{I assume $z=(x,y)$; but, did we define it earlier?}
%\notemg{$z_*, \xi_*$ in theorem below is not defined?.}
% Let $\xi_*^\top =[z_*^\top,z_*^\top]$. Given any $\varphi \in (0,1)$ and $M>0$ so that $\int_{\Vert z-z_*\Vert <M} p(\xi_*,z)dz\geq\sqrt{\varphi}$ and any given $R>0$ such that the following inequality holds 
% $$
% \inf_{\xi\in\mathbb{R}^{2d}, z\in\mathbb{R}^{d}, V(\xi)<R, \Vert z-z_*\Vert\leq M} \frac{p(\xi,z)}{p(\xi_*,z)}>\sqrt{\varphi}
% $$
% with the Lyapunov function,
\begin{multline}\label{def: lyap-func}
    \mathcal{V}(\xi_k)\sa{\triangleq}\frac{\theta}{1-\theta}\Big(\frac{\mu_x}{4}(\Vert x_k-x_*\Vert^2+\Vert x_{k-1}-x_*\Vert^2)+ \frac{\mu_y}{\sa{8}}(1+\theta)(\Vert y_k-y_*\Vert^2 + \Vert y_{k-1}-y_*\Vert^2)\Big),
\end{multline}
\mg{for which we can show that \eqref{cond-major-main-text} holds 
%with appropriate constants 
\sa{for some $\zeta\in(0,1)$ and $K\geq 0$} (see the appendix for more details). Then, building on the results of \cite{hairer2011yet}, we %obtain the following convergence rate 
\sa{\mg{establish in the following result} that the distributions of SAPD iterates converge to the invariant distribution, and also give a rate result for this convergence} provided that the variance of the gradient noise is not too large. \mg{The proof is deferred to the appendix}.}%
\begin{theorem}\label{thm: inv-meas-exists}  \mg{Consider the SAPD algorithm with parameters given by \eqref{eq:SAPD-parameters}. Suppose that Assumptions \ref{assump: obj-fun-prop}, \ref{assump: noise-properties} and \ref{assump-cont-density} hold, and} %under the setting of Proposition \ref{prop: conv-of-SAPD}. Suppose
%Suppose the noise admits a continuous probability density function in addition to 
%Assumption \ref{assump: noise-properties} holds. 
%\notemg{define the Lyapunov function $V$ either in the main text or in the theorem statement?}
the variance \bcred{bound} %$\tau_2$ 
\sa{$\delta_{(2)}^2$} of \mg{the noise is small} such that 
%enough so that the inequality}
\begin{equation}
%\delta_{(2)}^2
\sa{{(1+\theta)}\left(\frac{4}{\mu_x}+\frac{8}{\mu_y}\Big((1+\theta)^2+\theta^2\Big)\right)\delta_{(2)}^2}\leq R,
\end{equation}
%where $\bar{\rho}=\max\{ \theta(1+\tau \eta_x), \theta (1+(1+2\theta)\sigma \eta_y)\}$ for positive constants $\eta_x<\frac{1}{\tau}(\frac{1}{\theta}-1)= \mu_x$ and $\eta_y < \frac{1}{\sigma (1+2\theta)}\left(\frac{1+\theta}{2\theta}-1 \right)=\frac{\mu_y}{2+4\theta}$. 
%is satisfied 
where $R$ is a constant specified in the Appendix. Then \sa{for any initialization $\xi_0 \in \mathbb{R}^{2d}$,} SAPD iterates %starting from  
admit a %there exists a 
unique invariant measure %$\ptdt_*$
$\pi^{(\theta)}_*$, \sa{i.e., %for any initial distribution $\xi_0\sim\lambda$, 
$\lambda_{\xi_0}\mcR_k^{(\theta)}$, the distribution of \bcred{$\xi_k^{(\theta)}$}, converges to $\sa{\pi^{(\theta)}_*}$, where $\lambda_{\xi_0}$ denotes the Dirac distribution at $\xi_0$.} Moreover, there exists \sa{$C>0$} % \notemg{C is used before, call it $C_2$?}
such that 
$$
\Vert \sa{\mcR_k^{(\theta)}} \psi - \sa{\pi^{(\theta)}_*}(\psi)\Vert \leq \sa{C} %\bar{\rho}^k 
\sa{\left(\frac{2\theta}{1+\theta}\right)^k}\Vert \psi - \sa{\pi^{(\theta)}_*}(\psi)\Vert,
$$
%\todo{Burada direk $\pi^{(\theta)}$ diyebiliriz ayni sekilde $\mcR^{(\theta)}$.}
for \bc{any initialization $\xi_0$} and every measurable function $\psi$ such that $\Vert \psi \Vert <\infty$, where $\Vert \psi \Vert \triangleq \sup_{\xi} \frac{|\psi(\xi)|}{1+\mathcal{V}(\xi)}$ is the weighted supremum norm.
\end{theorem}
\mg{\sa{Since $\theta\in(\hat\theta,1)$,} by taking limit superior of both sides in \eqref{cond: SAPD-convergence-result} as $k\to \infty$, it can be seen that we have $$\limsup_{k\to\infty} \mathbb{E}[\|z_k - z_*\|^2] = \mathcal{O}(1-\theta)~\sa{\delta^2_{(2)}}.$$
%as $\theta \to 1$. 
Since the distribution of the SAPD iterates $z_k$ converges to the stationary distribution based on Theorem \ref{thm: inv-meas-exists}, we can replace the limit superieure with a limit to obtain $$\sa{\mathbb{E}[\|z_\infty - z_*\|^2] =} \lim_{k\to\infty}\mathbb{E}[\|z_k - z_*\|^2] =  \mathcal{O}(1-\theta)~\sa{\delta^2_{(2)}},$$
with the convention that $z_\infty$ is distributed according to the stationary distribution. This is summarized in Lemma \ref{lem: finite-moment} below, where we also characterize the fourth moments of the stationary distribution as a function of $\theta$ as $\theta \to 1$. In particular, obtaining the fourth moments require a careful non-trivial Lyapunov analysis of the SAPD algorithm that involves higher-order interactions between the gradient noise and the iterates; the proof is deferred to the appendix.
}

%The Lemma \ref{lem: finite-moment} shows that the invariant measure of Markov chain generated by SAPD has finite 4-th moment, if the noise in the algorithm admits Assumption \ref{assump: noise-properties}.
\begin{lemma}\label{lem: finite-moment}
\mg{%In the setting 
\sa{Under the premise} of Theorem \ref{thm: inv-meas-exists}, %we have 
$\mE[\Vert z_\infty-z_*\Vert^2]=\mathcal{O}(1-\theta)$ and $\mE[\Vert z_\infty-z_*\Vert^4]=\mathcal{O}\left((1-\theta\right)^2)$,
where $z_\infty$ is a random variable distributed according to the stationary distribution of the SAPD iterates.}
\end{lemma}
\mg{Building on this lemma, in the next result, we show that the expected iterates contain a bias that is %proportional to $1-\theta$ up to the first order 
\sa{$\cO(1-\theta)$} as $\theta \to 1$. The bias stems mainly from the fact that we use constant primal and dual stepsizes in SAPD as opposed to decaying stepsizes.} \bc{Our proof is based on relating the bias to the equilibrium covariance of the iterates and characterizing the equilibrium covariance as the solution to a set of coupled algebraic Lyapunov equations (whose solutions can then be approximated as $\theta\to 1$).}
\begin{theorem}\label{thm: expansion-at-inv-meas-mean}
%Let $f$ and noisy gradient estimates $\tn f$ admit the conditions of Theorem \ref{thm: inv-meas-exists}, in addition to satisfying Assumptions \ref{assump: obj-fun-prop} and \ref{assump: noise-properties}. 
%In the setting 
\sa{Under the premise} of Theorem \ref{thm: inv-meas-exists}, \sa{the limit of expected SAPD iterate sequence, i.e.,}
%consider the expectation of the iterates%
%hen, the distribution of the iterates $\{\xi_{k}^{(\theta)}\}_{k\in\mathbb{N}^+}$ \todo{Farkettim ki $\mathbb{N}^+$ is natural numbers+ 0 olarak define ettim ama bence yaniltici oldu onun yerine $\mathbb{N}$ diyip notation'da soyleyecegim} generated by SAPD converges to an invariant measure $\pi_{*}^{(\theta)}$.\footnote{We adapt the notations $\xi_{k}^{(\theta)}:=\xi_k^{(\tau,\sigma,\theta)}$ and $\pi_*^{(\theta)}:=\pi_{*}^{(\tau,\sigma,\theta)}$ for simplicity since the parameters only depend on $\theta$.} Moreover, the expected 
$$\bar{\xi}^{(\theta)}\triangleq\lim_{k\rightarrow \infty}\mathbb{E}[\xi_k^{(\theta)}],$$
\sa{exists} at stationarity %. We have the expansion
\sa{such that}
\begin{equation}\label{eq: inv-meas-mean}
    \bar{\xi}^{(\theta)}-\xi_*=(1-\theta)\bcred{\begin{bmatrix} (\hes)^{-1} \left( \nabla^{(3)}f_*M\right)\\
    (\hes)^{-1} \left( \nabla^{(3)}f_*M\right)
    \end{bmatrix}}+\mathcal{O}\left((1-\theta)^{3/2}\right),
    %+ \mathcal{O}\left((1-\theta)^2\right)
\end{equation}
as $\theta \to 1$
where \bcred{$\xi_{*}=(z_*,z_*)$,} $M$ is a fixed matrix \mg{with an explicit formula provided in the appendix}, \mg{$\hes$ is the Hessian matrix at the saddle point $z_*$, and $\nabla^{(3)}_*f$ is the tensor of order 3 that contains the third-order partial derivatives of $f$ at $z_*$.}
\end{theorem}
% Notice that under the setting of Proposition \ref{prop: conv-of-SAPD}, the SAPD algorithm \ref{alg: sapd} is given by single parameter $\theta$; therefore, we can adapt the notations $\xi_k^{(\theta)}\triangleq \xi_k^{(\tau_{\theta},\sigma_{\theta},\theta)}$, $\mcR^{(\theta)}\triangleq\mcR^{(\tau_\theta,\sigma_\theta,\theta)}$, and $\pi_*^{(\theta)}\triangleq \pi_{*}^{(\tau_\theta,\sigma_{\theta},\theta)}$.
\mg{Theorem \ref{thm: expansion-at-inv-meas-mean} shows that the expected iterates admit a bias that is $\mathcal{O}(1-\theta)$}. \mg{Following a similar approach to \sa{Richardson-Romberg} extrapolation techniques %developed 
\sa{adopted} for stochastic gradient descent methods \sa{for} unconstrained optimization in~\cite{bridging-the-gap}, %this 
\sa{our result in \eqref{eq: inv-meas-mean}} suggests that if we generate two SAPD sequence $\{\xi_k^{(\theta_1)}\}$ and $\{\xi_k^{(\theta_2)}\}$, then 
%we could scale the outputs of these sequences 
\sa{through appropriately forming a weighted sequence using the two, one can eliminate a significant portion of the bias.} 
%the sequence $\{2\xi_{k}^{(\theta_1)}-\xi_{k}^{(\theta_2)} \}$ can obtain better performance. Particularly, 
%For example, 
\sa{Indeed,} if we choose the parameters as $\theta_2=2\theta_1-1$, then the from \bcred{Theorem \ref{thm: expansion-at-inv-meas-mean}}, we obtain 
$$
2\bar{\xi}^{(\theta_1)}-\bar{\xi}^{(\theta_2)}= \xi_*+\mathcal{O}\left((1-\theta)^{3/2}\right),
$$}%
\sa{i.e., the bias improves from $\cO(1-\theta)$ to $\cO\left((1-\theta)^{3/2}\right)$.} \mg{That being said, the variance of $\{2\xi_k^{(\theta_1)}-\xi_k^{(\theta_2)}\}_k$ sequence could be larger than that of $\{\xi_k^{(\theta_1)}\}$. For controlling the variance, a standard idea in stochastic approximation methods is to consider the average of the iterates, \sa{i.e., consider $\{\tilde{\xi}_k^{(\theta)}\}_{k\in\mathbb{N}_+}$ such that for $k\geq 1$,} }
\begin{equation}
\bcred{\tilde{\xi}_k^{(\theta)}\sa{\triangleq} \frac{1}{k}\sum_{i=0}^{k-1}\xi_{i}^{(\theta)}}.
\label{def-aver-seq}
\end{equation}
\mg{Often, based on central limit theorem-type arguments, 
%it is the case that considering 
$\tilde{\xi}_k^{(\theta)}$ improves the variance of $\xi_k^{(\theta)}$ due to its \sa{averaged} nature. 

Next, in the following result, we study the gap between the mean of the averaged %sequence
\sa{iterate} $\tilde{\xi}_k^{(\theta)}$ and \bcred{$\bar{\xi}^{(\theta)}$} defined in Theorem \ref{thm: expansion-at-inv-meas-mean}}. The result shows that this gap decays polynomially fast in $k$ and is of the order $\mathcal{O}(1/k)$.

\begin{theorem}\label{thm: av-seq-conv}
\mg{%In the setting 
\sa{Under the premise} of Theorem \ref{thm: inv-meas-exists}, let $\xi_0$ be the initialization of the SAPD iterates
 $\{\xi_k^{(\theta)}\}_{k\in\mathbb{N}}$. %Given 
\sa{For any $\xi_0$ and \bcred{$k\geq 1$}}, %the following limit
% \begin{equation}\label{def: Psi^theta}
% \Psi^{(\theta)}\triangleq\lim_{k\rightarrow \infty}
% %\Psi_k^{(\theta)}\triangleq
% \sum_{i=0}^{k}(\mathbb{E}[\xi_{i}^{(\theta)}]\bcred{-\bar{\xi}^{(\theta)}}),
% \end{equation}
% exists. Moreover, we have
\begin{equation}\label{eq: gap-avg-mean-and-inv-meas-mean}
 \mathbb{E}[\tilde{\xi}_k^{(\theta)}]=\bar{\xi}^{(\theta)}+\frac{1+\theta}{1-\theta} \left(1-\left(\frac{2\theta}{1+\theta}\right)^k\right)\frac{C}{k}~\norm{\bcred{\xi_0-\bar{\xi}^{\theta}}},
% \mathbb{E}[\tilde{\xi}_k^{(\theta)}]-\bar{\xi}^{(\theta)}= \frac{1}{k}\Psi^{(\theta)}(\xi_0) + \mathcal{O}\left(\bcred{\frac{r^k}{k}}\right),
\end{equation}
where \sa{$C>0$ is the constant defined in Theorem~\ref{thm: inv-meas-exists}} and $\tilde{\xi}_k^{(\theta)}$ is the averaged %sequence 
\sa{iterate} defined in \eqref{def-aver-seq}}.
\end{theorem}
%\nsa{$\bar{\rho}$ olmamasi lazim yukardaki sonucta.}
From the equations \eqref{eq: inv-meas-mean} and \eqref{eq: gap-avg-mean-and-inv-meas-mean}, we obtain that  
\begin{equation}\label{eq: mean-av-seq}
\mathbb{E}[\tilde{\xi}_k^{(\theta)}]- \xi_* = %\frac{\Psi^{(\theta)}(\xi_0)}{k}
\sa{\frac{1+\theta}{1-\theta}~\frac{C}{k}\norm{\xi_0-\bar{\xi}^{\theta}}}+ (1-\theta) \bcred{\begin{bmatrix}(\hes)^{-1} \nabla^{(3)}f_*M\\(\hes)^{-1} \nabla^{(3)}f_*M \end{bmatrix}} + r_{\theta},
\end{equation}
where $\Vert r_{\theta}\Vert <C_3(1-\theta)^{3/2} + \sa{\tfrac{1}{k}} e^{-k C_4(1-\theta)}$ for some constants $C_3, C_4>0$. In particular, given that the error between $\mathbb{E}[\tilde{\xi}_k^{(\theta)}]$ and $\bar{\xi}^{\theta}$ is vanishing, 
we could apply the same variance reduction ideas to the averaged sequence \bcred{$\{\tilde{\xi}_k^{(\theta)}\}$} to reduce the variance. In the following section, we provide numerical examples to illustrate the benefits of our variance reduced SAPD method.
%\todo{Buraya SGDA ile ilgili bir seyler eklenebilir.}



